QUBIQ: Uncertainty Quantification for Biomedical Image Segmentation Challenge

Uncertainty in medical image segmentation tasks, especially inter-rater variability, arising from differences in interpretations and annotations by various experts, presents a significant challenge in achieving consistent and reliable image segmentation. This variability not only reflects the inherent complexity and subjective nature of medical image interpretation but also directly impacts the development and evaluation of automated segmentation algorithms. Accurately modeling and quantifying this variability is essential for enhancing the robustness and clinical applicability of these algorithms. We report the set-up and summarize the benchmark results of the Quantification of Uncertainties in Biomedical Image Quantification Challenge (QUBIQ), which was organized in conjunction with International Conferences on Medical Image Computing and Computer-Assisted Intervention (MICCAI) 2020 and 2021. The challenge focuses on the uncertainty quantification of medical image segmentation which considers the omnipresence of inter-rater variability in imaging datasets. The large collection of images with multi-rater annotations features various modalities such as MRI and CT; various organs such as the brain, prostate, kidney, and pancreas; and different image dimensions 2D-vs-3D. A total of 24 teams submitted different solutions to the problem, combining various baseline models, Bayesian neural networks, and ensemble model techniques. The obtained results indicate the importance of the ensemble models, as well as the need for further research to develop efficient 3D methods for uncertainty quantification methods in 3D segmentation tasks.

==> backup/old_tables.tex <==
% \section{Method descriptions.}
% %%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
\begin{landscape}
\begin{table}
\tiny
\caption{Details of the participating teams’ methods in QUBIQ-Challenge-2020 (part 1).} 
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{tabular}{l l l c c c c c c c c c }
\toprule
\tabincell{l}{\textbf{Lead Author} \& \\ \textbf{Team Members}} & \tabincell{l}{\textbf{Method, Architecture} \& \\ \textbf{Modifications}} & \tabincell{l}{\textbf{Data Augmentation}} & \textbf{Loss Function}  &\textbf{Optimizer Training} & \textbf{Pre-processing}  &\textbf{Label Processing} & \textbf{Ensemble strategy}\\
\midrule
\tabincell{l}{\crule[b0b0ff]{0.15cm}{0.15cm} \textbf{Jun Ma};}  & \tabincell{l}{2D U-Net\\one model per \\annotation.}  &  \tabincell{l}{None}  & cross-entropy and dice loss & None & \tabincell{l}{None} & \tabincell{l}{None} & \tabincell{l}{Ensemble with multiple models}\\
\midrule
\tabincell{l}{\crule[00b000]{0.15cm}{0.15cm} \textbf{Davood Karimi};}  & \tabincell{l}{2D U-Net with additional\\  connections between coarse and \\ fine feature layers in the\\ encoder. Dynamic weighting\\ of loss for harder classes.\\ Multi-task training approach.}  &  \tabincell{l}{None}  & 1-Dice similarity loss & None & \tabincell{l}{normalizing values with\\ 0 mean, unit\\ standard deviation.} & \tabincell{l}{labels with weight=1\\ for regions where\\ else ratio of \\agreement} & \tabincell{l}{None}\\
\midrule



\tabincell{l}{\crule[e4e400]{0.15cm}{0.15cm} \textbf{Ming Feng}; \\ Kele Xu, \\Yin Wang}  & \tabincell{l}{2D U-Net \\ Binarize ground truth\\\& predictions at different \\probability levels.\\ \& average dice score of\\each prediction}  &  \tabincell{l}{Random scaling \\(0.9 -- 1.1)}  & \tabincell{l}{weighted cross entropy \\ and dice}  & Adam & \tabincell{l}{Brain Tumor: resize \\ to 256 $\times$ 256.\\ kidney \& prostrate \\512 $\times$ 512. \\Normalize data in 0-255} & \tabincell{l}{labels with weight=1\\ for regions where\\ else ratio of \\agreement} & None\\
\midrule

\tabincell{l}{\crule[baba00]{0.15cm}{0.15cm} \textbf{Raghavendra Selvan}}  & \tabincell{l}{Multi-channel U-Net. \\One channel for each rater.\\Based on idea of \\ Normalizing Flows}  &  \tabincell{l}{None}  & \tabincell{l}{Planar Flow \\ \& dice loss}  & None & \tabincell{l}{None} & \tabincell{l}{None} & \tabincell{l}{None}\\
\midrule

\tabincell{l}{\crule[008900]{0.15cm}{0.15cm} \textbf{Ujjwal Baid}; \\ Prasad Dutande, \\Shubham Innani, \\ Bhakti Baheti, \\Sanjay
Talbar}  & \tabincell{l}{ResNet34 based encoder-decode.\\Different ground truths \\ are included in training\\set as individual copies.}  &  \tabincell{l}{rotation, flips \& scaling}  & None & None & \tabincell{l}{Brain:Resizing images\\ to 256 $\times$256\\kidney: resizing to 512 $\times$512 \\Prostrate: resize 640 $\times$640.} & \tabincell{l}{None} & \tabincell{l}{None}\\
\midrule

\tabincell{l}{\crule[545400]{0.15cm}{0.15cm} \textbf{Wesam Adel}; \\ Mustafa A. Elattar}  & \tabincell{l}{2D U-Net\\Different expert annotations\\averaged to create \\training labels. Treated as a \\regression problem.}  &  \tabincell{l}{None}  & weighted kl-divergence & None & \tabincell{l}{Brain: Resize to \\256 $\times$ 256\\with rotation and elastic\\deformaation.} & \tabincell{l}{None} & \tabincell{l}{None}\\
\midrule

\tabincell{l}{\crule[00ff00]{0.15cm}{0.15cm} \textbf{Xiang Li};}  & \tabincell{l}{U Net with attention\\ 4 downsampling for Kidney\\and 5 for others}  &  \tabincell{l}{None}  & weighted cross entropy & Adam & \tabincell{l}{Kidney: Cropped to 128$\times$128.\\Prostrate:Cropped to 416$\times$416} & \tabincell{l}{labels with weight=1\\ for regions where\\ else ratio of \\agreement} & \tabincell{l}{None}\\
\midrule
\tabincell{l}{\crule[550500]{0.15cm}{0.15cm} \textbf{Yanwu Yang}; \\ Ting Ma}  & \tabincell{l}{2D U-Net with multiple \\branches. Instance Norm \\used instead of \\Batch Norm. One model per\\annotation and integrated \\using auxiliary loss}  &  \tabincell{l}{None}  & Dice \& cross entropy & Adam & \tabincell{l}{MRI:z-score normalization.\\CT: focus on ROI\\and rescale to [0 -- 1]} & \tabincell{l}{None} & \tabincell{l}{Averaging}\\
\midrule
\tabincell{l}{\crule[00b0b0]{0.15cm}{0.15cm} \textbf{Wei Ji}; \\ Wenting Chen\\Shuang Yu\\Kai Ma\\Li Cheng\\Linlin
Shen\\Yefeng Zheng}  & \tabincell{l}{U-Net with Resnet-34 \\encoder. One output \\channel per label. \\Batch Norm. One model per\\annotation and integrated \\using auxiliary loss}  &  \tabincell{l}{None}  & cross entropy & Adam & \tabincell{l}{Resize to \\512 $\times$512} & \tabincell{l}{Both fused\\final \& individual\\labels. Three techniques\\to combine labels\\average, random and\\label sampling.} & \tabincell{l}{Sum of \\weighted predictions.}\\

\bottomrule
%    \midrule
\end{tabular}
\label{tab:method_1}
\end{table}
% \caption{Details of the participating teams’ methods.}

\end{landscape}
\end{center}
% \clearpage



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%
%\begin{center}
\begin{landscape}
\begin{table}
\tiny
\caption{Details of the participating teams’ methods in QUBIQ-Challenge-2021 (part 2).}  
\setlength\tabcolsep{4pt} % default value: 6pt

\begin{tabular}{l l c c c c c c c c c c }
\toprule
\tabincell{l}{\textbf{Lead Author} \& \\ \textbf{Team Members}} & \tabincell{l}{\textbf{Method, Architecture} \& \\ \textbf{Modifications}} & \tabincell{l}{\textbf{Data Augmentation}} & \textbf{Loss Function}  &\textbf{Optimizer Training} & \textbf{Pre-processing}  &\textbf{Label Processing} & \textbf{Ensemble strategy}\\
\midrule


\tabincell{l}{\crule[00b000]{0.15cm}{0.15cm}  \textbf{Anindo Saha};\\ Henkjan Huisman}  & \tabincell{l}{Probabilistic U-Net}  & \tabincell{l}{Gaussian noise\\horizontal flip\\rotation\\translation , scaling} & \tabincell{l}{KL-Divergence and \\Dice loss}  & AMSGrad & \tabincell{l}{z-score normalization\\ Centre crops with \\Kidney: 512 $\times$512\\Brain: 256$\times$256 \\Prostrate: 640$\times$640}& None & \tabincell{l}{MC Dropout on \\individual U-Net \\and \\Deep ensemble \\(averaging)}\\[-2pt]

\midrule


\tabincell{l}{\crule[e4e400]{0.15cm}{0.15cm} \textbf{Hoang Long Le}; \\Jin Tae Kwak}  & \tabincell{l}{DeepLabv3 and \\Efficientnet with latter\\used for classification.\\ 9 binary ground\\truth by\\thresholding. \\Classification to check\\pancreas existance\\in image} & \tabincell{l}{horizontal \& vertical \\flip, rotate, shift\\scale, Gaussian noise\\blur, random \\brightness. }& Dice loss &  Adam& \tabincell{l}{0$--$1 normalization\\ and multiplied by \\255} &\tabincell{l}{Average of \\annotations} & \tabincell{l}{Multiply binary\\segmentation map with\\threshold value \& \\take per pixel\\maximum.} \\ [-2pt]
\midrule
\tabincell{l}{\crule[baba00]{0.15cm}{0.15cm} \textbf{Ishaan Bhat};\\Hugo J. Kuijf } & \tabincell{l}{Probabilistic U-Net \\with MC Dropout}   & \tabincell{l}{random flip,\\rotation, \\brightness \& \\contrast}&\tabincell{l}{cross entropy \&\\ KL-Divergence}& Adam & \tabincell{l}{z-score normalization\\Resize Brain: 256$\times$256\\Kidney: 512$\times$512\\Pancreas: 512$\times$512} & \tabincell{l}{None} & \tabincell{l}{Deep ensemble \\(averaging)} \\ [-2pt]
\midrule


% New changes start
\tabincell{l}{\crule[00b000]{0.15cm}{0.15cm}  \textbf{Dewen Zeng}; \\ Yukun Ding\\Yiyu Shi}  & \tabincell{l}{2D U-Net\\with multiple loss\\functions. One for the \\individual annotators, \\one on the aggregated label\\\& one on multi-scale\\threshold}  & \tabincell{l}{None} & \tabincell{l}{Cross Entropy}  & \tabincell{l}{z-Score normalization,\\ resizing} & \tabincell{l}{Averaging annotations} & \tabincell{l}{None}\\[-2pt]
\midrule

\tabincell{l}{\crule[00b000]{0.15cm}{0.15cm}  \textbf{Yanwu Yang}; \\ Xutao Guo\\Yiwei Pan\\Pengcheng Shi\\Haiyan Lv\\Ting Ma}  & \tabincell{l}{2D U-Net\\with multiple decoders,\\one for the \\individual annotators. The U-Net is modified to \\have Layer Norm and \\skip-connections in the\\individual encoder-decoder blocks.}  & \tabincell{l}{None} & \tabincell{l}{Cross Entropy \& Dice loss\\on individual decoders\\A cross loss between\\different decoders \\\& an auxiliary loss between average \\prediction \& average ground truth}  & \tabincell{l}{z-Score normalization,\\ resizing} &\tabincell{l}{Averaging different labels} & \tabincell{l}{Deep ensemble \\ (averaging)}\\[-2pt]
\midrule

\tabincell{l}{\crule[00b000]{0.15cm}{0.15cm}  \textbf{Stephan Huschauer};}  & \tabincell{l}{High-Resolution Network (HRNet)\\ with stem layers replaced by\\ 2D wavelet scattering transformation}  & \tabincell{l}{None} & \tabincell{l}{None}  & \tabincell{l}{Resize to 512 $\times$ 512}&\tabincell{l}{Averaging annotations} & \tabincell{l}{Deep ensemble \\ (averaging)}\\[-2pt]
\midrule

\tabincell{l}{\crule[00b000]{0.15cm}{0.15cm}  \textbf{Xiaofeng Liu};\\Fangxu Xing\\Georges El Fakhri\\Jonghye Woo}  & \tabincell{l}{Variational Inference\\ with encoding multi-\\annotator variability using\\latent variable model.}  & \tabincell{l}{None} & \tabincell{l}{Cross Entropy \\\& L2 reconstruction loss}  & \tabincell{l}{None}&\tabincell{l}{Averaging annotations} & \tabincell{l}{Deep ensemble \\ (averaging)}\\[-2pt]
\midrule

\tabincell{l}{\crule[00b000]{0.15cm}{0.15cm}  \textbf{Yucong Chen};\\Guanqi He\\Zhitong Gao\\Xuming He}  & \tabincell{l}{2D U-Net\\with multiple decoders,\\one for the\\individual annotators.}  & \tabincell{l}{Training: Random crop\\Inference: Sliding Window} & \tabincell{l}{None}  & \tabincell{l}{None}&\tabincell{l}{None} & \tabincell{l}{Deep ensemble \\ (averaging)}\\[-2pt]
\midrule

\tabincell{l}{\crule[00b000]{0.15cm}{0.15cm}  \textbf{Timothy Sum Hon Mun};\\Simon J Doran\\Paul Huang\\Christina Messiou\\Matthew D Blackledge}  & \tabincell{l}{2D U-Net with \\Monte Carlo dropout.}  & \tabincell{l}{None} & \tabincell{l}{Dice loss}  & \tabincell{l}{None}&\tabincell{l}{None} & \tabincell{l}{None}\\[-2pt]
\midrule

% New changes end

\tabincell{l}{\crule[008900]{0.15cm}{0.15cm} \textbf{Jiachen Zhao};} & \tabincell{l}{U-Net}   & \tabincell{l}{random flip}&\tabincell{l}{Dice loss}& Adam & \tabincell{l}{Resize images to\\256 $\times$ 256} & \tabincell{l}{Average of\\annotations} & \tabincell{l}{None} \\ [-2pt]
\midrule
\tabincell{l}{\crule[545400]{0.15cm}{0.15cm} \textbf{Jimut Bahan Pal};} & \tabincell{l}{U-Net \\One model per\\annotator}   & \tabincell{l}{None}&\tabincell{l}{Focal Tversky}& Nadam & \tabincell{l}{None} & \tabincell{l}{None} & \tabincell{l}{None} \\ [-2pt]
\midrule
\tabincell{l}{\crule[00ff00]{0.15cm}{0.15cm} \textbf{Jo\~ao Louren\c{c}o Silva};\\Arlindo L. Oliveira} & \tabincell{l}{U-Net with\\ EfficientNet-B0 \\encoder.}   & \tabincell{l}{rotation, translation\\zoom, horizontal\\\& vertical flips.}&\tabincell{l}{cross-entropy}& Adam & \tabincell{l}{None} & \tabincell{l}{Averaging of\\ segmentation maps} & \tabincell{l}{None} \\ [-2pt]
\midrule
\tabincell{l}{\crule[550500]{0.15cm}{0.15cm} \textbf{Martin \~{Z}ukovec};\\Lara Dular\\\~{Z}iga \~{S}piclin} & \tabincell{l}{nnU-Net. Treating task\\as multi-class\\classification with labels\\ 0--N where 0 \\is background and \\N is number of annotators.}   & \tabincell{l}{rotation, scaling\\mirroring, inhomogeneity\\\& Gaussian noise.}&\tabincell{l}{Dice loss}& SGD + Momentum & \tabincell{l}{image sampling\\and normalization} & \tabincell{l}{Addition of\\ individual\\ segmentation maps} & \tabincell{l}{None} \\ [-2pt]
\midrule
\tabincell{l}{\crule[00b0b0]{0.15cm}{0.15cm} \textbf{Sabri Can Cetindag};\\M ert Y ergin\\Deniz Alis \\Ilkay Oksuz} & \tabincell{l}{nnU-Net. Two stage\\training. Obtaining individual\\U-Net models per\\annotator \& adding\\segmentation map output\\as extra channels\\in the second\\stage}   & \tabincell{l}{None}&\tabincell{l}{cross entropy \\ \& Dice loss}& SGD + Nestrov & \tabincell{l}{None} & \tabincell{l}{Average of\\ individual\\ segmentation maps\\for stage 2} & \tabincell{l}{None} \\ [-2pt]
\midrule
\tabincell{l}{\crule[888700]{0.15cm}{0.15cm} \textbf{Xiong Wang};\\Shengbo Gao\\Weifeng Hu\\Xuan Pei} & \tabincell{l}{2D: U-Net, MaskNet, \\ and DeepLab V3+.\\3D: SegResNet\\ Obtaining individual\\U-Net models per\\annotator trained using\\label fudion strategy}   & \tabincell{l}{None}&\tabincell{l}{weighted Focal\\ \& Dice loss}& SGD + Nestrov & \tabincell{l}{None} & \tabincell{l}{label fusion\\for training\\individual models.} & \tabincell{l}{weighted combination\\of individual\\predictions} \\ [-2pt]
\midrule
\tabincell{l}{\crule[ff00ff]{0.15cm}{0.15cm} \textbf{YingLin Zhang};\\Wei Wang\\Ruiling Xi\\Lingxi Zeng\\Huiyan Lin} & \tabincell{l}{UNet, UNet++,\\ and TransUNet}   & \tabincell{l}{random flip,\\
random brightness,\\ sharpness, and contrast change.\\Random blur, random noise,\\ random shift, zoom,\\ random rotation, and ''elastic transformation.}&\tabincell{l}{multiple-level \\Dice los}& SGD + Momentum & \tabincell{l}{Crop images \\ so that ROI\\is at the centre.\\Discard images if ROI \\not clear enough} & \tabincell{l}{Three strategies:\\majority voting,\\ cumulative
division\\ and even division  of\\ individual\\ segmentation maps} & \tabincell{l}{weighted combination\\of individual\\predictions} \\ [-2pt]
\midrule

\tabincell{l}{\crule[ff0000]{0.15cm}{0.15cm} \textbf{Yingbin Bai};\\Maoying Qiao\\Dadong Wang\\Tongliang Liu} & \tabincell{l}{UNet++ with \\EfficientNet-B7 encoder.\\}   & \tabincell{l}{None}&\tabincell{l}{multiple-level \\Dice los}& SGD + Momentum & \tabincell{l}{None} & \tabincell{l}{weighted combination\\of individual\\segmentation maps} & \tabincell{l}{None} \\ [-2pt]
\midrule

\bottomrule
%    \midrule
\end{tabular}
\label{tab:method_2}
\end{table}
% \caption{Details of the participating teams’ methods.}
\end{landscape}
%\end{center}
